hSMAL: Detailed Horse Shape and Pose Reconstruction for Motion Pattern Recognition

In this paper we present our preliminary work on model-based behavioral analysis of horse motion. Our approach is based on the SMAL model, a 3D articulated statistical model of animal shape. We define a novel SMAL model for horses based on a new template, skeleton and shape space learned from $37$ horse toys. We test the accuracy of our hSMAL model in reconstructing a horse from 3D mocap data and images. We apply the hSMAL model to the problem of lameness detection from video, where we fit the model to images to recover 3D pose and train an ST-GCN network on pose data. A comparison with the same network trained on mocap points illustrates the benefit of our approach.

==> section/background.tex <==
\section{Background}
In this section, we describe some background that we used. The SMAL model and the process of reconstruction are introduced first. Then it comes up with the ST-GCN method. 

\subsection{SMAL model}
The SMAL model is proposed for five different quadruped families. It is a parametric model that can describe the shape and pose of the animal separately. The mean template is obtained from 41 different toy\mr{s'} data. The shape and pose are controlled by shape parameter $\beta$ and pose parameter $\theta$, respectively. The $\beta$ mainly defines the vertex deformation applied to the mean template. The specific-subject model can be expressed as Equation \ref{equa:specific model}
\begin{small}
\begin{center}
\begin{equation}
V(\beta) = V_{template} + B_s \beta
\label{equa:specific model}
\end{equation}
\end{center}
\end{small}
where $B_s \beta$ represents the difference between the specific subject and the mean template, and $B_s$ is a novel basis obtained by Principle Component Analysis. Pose parameter $\theta$ describes the relative rotation between different body parts and it follows a predefined kinematic tree in the model. The pose variable of the root joint $\theta_{root}$ in the kinematic tree denotes the global rotation and the global translation $\gamma$ applied on the root. 

\subsection{Fitting model to data}
The paper \cite{zuffi20173d} define an objective function to minimize when fitting the SMAL model to the image and annotated 2D keypoints. The function consists of different energy terms that limit the model from both shape and pose perspectives. Moreover, the energy terms are calculated from the 2D key points, silhouette, and model prior knowledge. More details are shown in Section \ref{sec:energyterm}.


% \ci{will delete, mentioned in related work} The SMPL model is learned from thousands of real human scans, and it can also capture the soft-tissue motion on the human body. The motion capture system records the movement of humans through a limited number of markers on the human body. The markers are distributed sparsely on rigid joints and non-rigid soft-tissue. Since the marker positions are difficult to stay on the fixed positions on the human body when humans are moving, MoSh first optimizes the marker position on the human model from the predefined marker vertexes. Then, MoSh fits the SMPL model to motion capture data with an objective function that mainly minimizes the distance between the markers and the human model. 

\subsection{ST-GCN}

ST-GCN \cite{yan2018spatial} emphasizes the importance of dynamic skeleton for human action recognition by taking the spatial and temporal information of joints into consideration. The whole framework consists of several ST-GCN blocks and each block consists of an attention layer for describing the important edges and a spatial graph convolution followed by a temporal graph convolution. A fully connected layer is connected to the last block for classification. Based on the convolution operation on the image, the author modified the sampling function and the weight function to adapt to skeleton data with multiple frames. The sampling function only samples the neighbors to the root node with one length. The weight function assigns different weights to neighbor nodes. 

==> section/instruction.tex <==
\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confYear~web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section,
must be no longer than eight pages in length. The references section
will not be included in the page count, and there is no limit on the
length of the references section. For example, a paper of eight pages
with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confYear.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.  

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. 
(\LaTeX\ users may use options of cvpr.cls to switch between different 
versions.)  
Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $095.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
techreports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors14} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors14b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the CVPR70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``
   Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
\cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.
%
Page numbers should be in footer with page numbers, centered and .75
inches from the bottom of the page and make it start at the correct page
number rather than the 4321 in the example.  To do this fine the line (around
line 20)
\begin{verbatim}
\setcounter{page}{4321}
\end{verbatim}
where the number 4321 is your assigned starting page.



%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confYear~web page for a discussion
of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.


==> section/literature_review.tex <==
\section{Literature Study}

% abnormal activity detection
% skeleton based approch
% pose estimation
%  reconstruction models
% sensor and camera based techniques

\subsection{Animal Lameness Detection}

\textbf{Paper \cite{9216873}} does lameness detection of horses based on the acceleration data collected from wearable IMU-based sensors. The data post-processing extracts gait cycle routines(GCPs) from the IMU data for the head angle to segment each trial. Each classifier in the multi-layer classifier (MLC) is designed independently for each binary classification task for walking and trotting, ordinary or lameness, left limb or right limb. 

Paper \cite{article} collects data by mounting sensors on sheep. First, the signals extracted from the sensors are defined as the root sum squared of the acceleration and gyroscope signals in three axes. The feature characteristics are obtained by computing the difference in the magnitude of the acceleration and the magnitude of the gyroscope, which measures the signals' change. Different classification algorithms like RF, NN, SVM, AdaBoost, and KNN are used to perform lameness detection. Each classifier models one activity among three activities(walking, standing, lying). 

Paper \cite{muller2020riding} does gait analysis of horses for lameness assessments based on the asymmetry movement of the head and pelvis and weight-bearing asymmetry. The paper compares the diagnoses by objective and subjective analysis and points out that subjective analysis is necessary and even two kinds of subjective statiscal analysis doesn't behave uniformly and needed to be considered carefully. 

Paper \cite{taneja2020machine} builds an end-to-end IoT application that combines the sensors on a dairy herd, a cloud computing system, a software for farmer to monitor the cows in real-time. The accelerometric data collected from sensors are transferred to a fog node for preproccssing and those data are used for data analysis by machine learning to detect lameness at the early stage.

\subsection{Human gait recognition}

Paper \cite{balazia2017human} uses the distance between two legs to extract gait cycle and picks up two particular poses as the signature poses. The pattern descriptor consists of twenty-one joints angles from the selected two signature poses using Mocap data. The Mocap data are first reprocessed to have same coordinate system. The identity classification performs by 1-NN classifier.

Paper \cite{balazia2018gait} learns the gait features by MMC, PCA+LDA from the between- and within-class and total scatter matrices of the 3D spatial coordinates of joints (motion capture data) of different identities. The authors compose a database with different templates for each person by extracting he/her gait features. When it comes to a new test person, the proposed framework calculates the similarity of the new gait feature with all the templates stored in the database and reports the most similar identity.

Paper \cite{horst2019explaining, slijepcevic2020explanation} emphasizes the uniqueness of gait patterns for individuals. Two kinds of data are recorded: lower-body joint angle in the sagittal plane(flexion-extension) (LBJAX) and ground reaction forces (GRF). The data are normalized by time as the input to DNNS for predicting different subjects. \textbf{The layer-Wise Relevance Propagation(LRP) is used for prediction interpretation, which explains the unique feature corresponding to the subject or contradicting the subject.}

Paper \cite{xugait} proposes a framework to do gait recognition based on the reconstructed whole gait cycle only given an arbitrary silhouette. The proposed framework PA-GCRNet contains PA-GCR for reconstruction and GaitSet for recognition.  

Paper \cite{li2020end} proposes an end-to-end method that recognize the gait based on 3D human model sequence instead of silhouette or skeletons that are used in existing approaches. The 3D human extraction use a pretrained network HMR. \textbf{The concatenation of 3D/2D joint locations on 3D sequences are used for feature extractions} through a CNN or LSTM and the triplet loss is used to minimize the distance of the same object and maximize the distance between different subjects.

Paper \cite{gu2010action} captures the 3D human joint and pose informatino using a markerless pose recovery method. Three movement features (position, orientation and height) are used for HMM model for action recognition. and two configuration features (normlaized joint position and upper limb) are used for EHMM model for gait recognition.

\textbf{Paper \cite{switonski2011human}} uses the motion capture system to obtain the human skeleton sequence by processing the mocap data with a defined skeleton model to estimate the pose. The joint angles are reduced by PCA technique. Fourier transform with low pass filtering is also applied in the feature extraction stage. Two statistical classifiers (kNN and NB) are selected.

\textbf{Paper \cite{krzeszowski2012view}} presents a view-independent gait recognition algorithm based on a 3D articulated body model. The algorithm capture the human motion in a markerless condition and four synchronized cameras and is evaluated by comparing the accuracy to Mocap system. Three aspects of data about the estimated human body (all joint angles, distance between ankles adn the height of the person) are considered. The data is analysed by multilinear PCA after normalization and segmentation into gait cycle. The new features are used for classification by NB and MLP classifiers.

\textbf{Paper \cite{fang2020gait} presents the gait neural network  (GNN) for both gait recognition and gait prediction.} GNN consists of two temporal convolutional network (TCN). TCN can handle the long range sequence-model tasks better with more flexibility when comparing to LSTM and the convolutions are causal. The dataset HuGaDB dataset contains gait data collected from inertial sensors. The first network is used to predict intermediate data and the predicted data is concanentated with the original input as the input to the second network. The idea aims to increase the number of learned feature and to obtain more historical information. The two fully connective layers are added to the final part for gair recognition and prediction. The acceleration shows periodic and similarity between different invididuals. 

Paper \cite{zou2020deep} does gait recognition by collecting IMU gait data from smart phones under unconstrained conditions. IMU gait data are six-dimensional sequences which consist of three dimensions of acceleration data and gyroscope. A segmentation algorithm with 1DCNN is used to segment the walking data from the entire data sequence which includes nonwalking data and thenn the gait cycles are segmented by selecting the acceleration data as the basis for partitioning. A CNN and a LSTM network is trained respectively and concatenated at the final layer to generate robust features in spatial and temporal domains for subject identification. For gait authentication, the CNN trained previously is used for feature extraction. Two input sequences extracts the same features in same structure by using the CNN and then the features are fed into the LSTM for authenticating whether two inputs are from the same person or not.

\subsection{Human gait analysis} 

Paper \cite{sandau2014markerless} proposes a novel approach to reconstruct the human body using the synchronized cameras without any attached markers on the subject. The statistical analysis of the pose data is done by comparing the results of the 3D reconstructed data and the marker-based system. The results show that this motion capture system can provide reliable human poses on different gait information. 

Paper \cite{gholami2020estimating} proposes only to use one accelerometer to estimate the joint angle by CNN. The data includes two parts: the joint angle calculated by the Vicon system, which records markers trajectories and acceleration data by a shoe-mounted accelerometer. A Butterworth low-pass filter is used to filter two kinds of data. A 1-D CNN is designed for estimating the joint angle from only the acceleration. The experiments are set up for the inter-participant method (splitting the data into training and test following a leave-one-person-out(LOSO) cross-validation scheme for inter-participants) and intra-participant method (80\% of data was randomly selected for training and the remaining 20\% for the test).

\subsection{Gait stride detection}

Paper \cite{anwary2018optimal} proposed a algorithm for automatically extract the gait features from raw IMU sensors. The features can be used for analysing speed, different stages in a gait cycle. The build-in function (findpeaks) in MATLAB is used to estimate the local maximal peak in the data vector which could help to estimate the stride number. 

Paper \cite{han2019gait} detects different stages in gait cycles by using IMU sensor data attached to the shank and Forse sensitive resistor (FSR). The gait cycle extraction is done by the maximum swing of the shanks. One cycle starts in a maximum swing and end up with a subsequence maximum swing. 
Paper \cite{gu2018markerless} reconstructs 3D joint positions of human lower limbs by using a RGB camera. The dorsiflexion/plantarflexion and inversion/eversion are extracted based on angle of the foot with the vertical image plane axis and horizontal image plan axis, respectively. The gait features also include foot progression angle and 3D foot-leg angle. The time series are segmented by Singular Spectrum Analysis (SSA).    

\subsection{Human abnormal gait analysis}

Paper \cite{khokhlova2018kinematic} uses the Cosine Rule to calculate the hip and knee flexion angles. And then the authors proposeto use covariance matrices based on the low-limb flexion as the gait feature. The detection strategy is different. A statistical normal gait model is selected when training data only contains normal data, otherwise K-NN classifier is used. The descriptor shows that the prior temporal segmentation is not necessary in this case.

Paper \cite{caramia2018imu} extracts the range of motions (RoMs) and the spatio-temporal parameters from raw data obtained from IMU sensors. Six different ML techniques are applied to different groups of features. And the results show that the combination of RoMs and spatio-temporal parameters leads to higher accuracies.

Paper \cite{esfahani2019using} uses an STS system comprised of smart socks and a smart shirt. The collected data are processed with Butterworth filters and are used to classify normal gait and four simulated gait abnormalities. Diverse modeling approaches like KNN, LDA, SVM, ANN are used.

Paper \cite{bauckhage2009automatic} proposes a novel homeomorphism that describes the silhouette of human in a walking sequence. The authors use SVM to detect unusual movement patterns. The results show that the new features can be reliably used for detecting some abnormal gaits like wavering, faltering and falling.

Paper \cite{li2018classification} uses an improved gait descriptor invariant to the walking cycles to process the skeleton data recorded by Kinect. The descriptor first calculates the positional covariance matrix to record the mutual joint positions along time and encodes the joints' relative speeds into another covariance matrix to have a better representation of the motion. The covariance matrix distance metric is defined to learn the gait similarity by concatenating two matrixes, and it is used for the KNN classifier to distinguish three gait classes (normal, Hemiplegic, and Parkinson).

\textbf{Paper \cite{khokhlova2019normal}} does gait analysis and classification between normal, limping, and knee rigid gait. The gait analysis calculates the flexion and rotation angles on low-limbs joints (specifically knee and hip) from the orientation data obtained from Kinect v.2 sensors and segments the gait sequence into cycles. The classification model is a single LSTM model and an ensemble LSTM model. 

\textbf{Paper \cite{gotlinautomated}} predicts the Gait Deviation Index(GDI), which indicates the gait pathology level (0-100) of the patients by only using 2D video. DensePose is applied to the raw video, aiming to map the pixels in 2D images to a 3D human model mesh. UV coordinates and PartIndex are extracted to represent the pixel locations on the human body (SMPL). A CNN is applied to these processed data, and a temporal model (LSTM) is added to capture the temporal information. 

Paper \cite{mallikarjuna2019feedback} focuses on identify abnormal gait caused from neurological disorders (parkinson/ neuropathic/ hemiplegic). The gait abnormalities mainly comes from the irregular patterns of the lean angle and ramp angle in three abnormal gaits compared to normal gait. 

\textbf{Paper \cite{nguyen2016skeleton}} proposes to build a model based on normal gaits and uses this model to detect abnormal human gait. The model is based on discrete HMM learning from human 3D skeleton sequences, and a test sequence with the lower expected likelihood output can be seen as an abnormal sequence. The data are processed to extract the features of low body joints, and the features are discretized into codewords by using K-means and separated into gait cycles. The HMM model is chosen for the effectiveness and the capability to represent unfixed sequence length. The expected threshold is estimated based on the log-likelihood of all training samples.

Paper \cite{chaaraoui2015abnormal} proposes joint motion history features (JMH) which encodes the temporal and spatial information about 3D locations of the skeleton sequence. The input skeleton sequences are normalized for  location, body size and rotation. The classification is done by BagOfKeyPoses method where the abnormal motion can be found in a learned normal model by a predefined threshold.

Paper \cite{nguyen2019applying} estimates the human gait abnormality index from 3D information. The 3D point clouds are obtained from multi-view points and represented by cylindrical histograms frame by frame. The adversarial auto encoder (AAE) is trained on normal data and the abnormal gaits are pointed out with the weighted sum of loss of the AE output, probability of a normal prior distribution and the discriminator output.  

Paper \cite{malik2020deep} utilizes micro-electro-mechanical motion sensors and electromyograph (EMG) system to collect multimodal biosignals. An autoencoder is trained on all normal gait data to estimate the normal distribution. The best model with a defined threshold can be used to detect abnormal gait when the reconstruction loss is larger than the throushold.

Paper \cite{gao2019abnormal} first fuses the gait data by using dynamic step conjugate gradient algorithm. And then the authors segment the calculated attitude by the similarity comparison between data segments and fitting the leg Euler angle to the proposed long short-term memory network and convolutional neural network (LCWSnet) for abnormal gait detection.

Paper \cite{gatt2019detecting} focuses on training a LSTM-AE and 1DConv-AE network inspried by \cite{malhotra2016lstm} on normal skeleton behavior extracting from Openpose and PoseNet. The framework considers three LSTM/ 1DConv layer (first layer for encoder, middle one for saving latent information and the last one for decoder). The abnormal sequences are recognized by being processed to the model by a threshold. 

Paper \cite{potluri2019deep} utilizes a plantar pressure measurement unit and IMU sensors to collect foot data and detect human gait abnormalities by an LSTM model based on the different regions which represent pressure on the feet. Only the normal data is used for training by minimizing the mean-squared-error loss between the ground-truth and the predicted subsequence. 

\textbf{Paper \cite{gu2020cross}} emphasis the importance to have pattern-specific features that is invariant to subject and data modal in abnormal gait recognition. The proposed architecture disentangles the pattern and subject specific representation by minimizing a set of predefined loss in reconstructing cross-subject patterns. Furthermore, the architecture also considers multi modal transfer between mocap data, RGBD data and EMG data.

Paper \cite{guo20193} estimates 3-D canonical pose and \textbf{extracts the joint angles as the features} and adopts two kinds of classifiers (SVM classifier for statistical features and Bi-LSTM classifier for angle sequences). For testing samples, the final prediction considers the voting results of all segments with the maximum occurrence frequency. 

Paper \cite{rueangsirarak2018automatic} makes diagnosis on disorder based on the motion capture data. The data are first converted to skeleton data and extracted the gait cycle through dynamic time warping. The proporsed 3D Relative Joint Displacement(3DRJDP) and the 6D Symmetric
Relative Joint Displacement (6DSymRJDP) can handle the relationship of joint pairs and used for classification by SVM. 

\subsection{Graph Convolution network}
Paper \cite{yan2018spatial} performs action recognition by a spatial-temporal gragh convolutional networks (ST-GCN) based on skeleton data. Paper \cite{shi2019two} points out the fixed topology of graph in ST-GCN and has more investigation on the second-order information of the skeleton. The authors proposes two-stream adaptive graph convolutional network (2s-AGCN) to improve the performance of ST-GCN. 

Paper \cite{hu2019vision} proposes an architecture that fuses the prediction of GCNN and context models to detect abnormal gait based on video. The GCNN consists not only graph convolution layer to describes the relation between different joint, but also \textbf{an adjacency matrix} to estimate the weight of each edge.

Paper \cite{li2019actional} proposes actional-structural graph convolution network (AS-GCN) that the structural links capture the dependencies between the joints inside the skeleton and the actional links denotes the relation of joint caused by the specific actions. An Encoder-decoder structure is applied so that the framework can both predict and recognize the action. 

Paper \cite{}  proposes Spatial Temporal Graph Convolutional Networks for Emotion Perception from Gaits (STEP) based on ST-GCN and CVAE. The network includes a gait generation network trained with real-human skeleton and a classification network for emotion classification. 

\subsection{extra from 2d recover 3d inform}

Paper \cite{balazia2017human, d2020markerless, juri2020characterization} estimate the 3D joint coordinates by using 2D information like mapping 2D joint extracted from Openpose to 3D joints through camera calibration. The final 3D joints can be used for gait analysis by estimate the rotation between joints, the joint angle. 

Paper \cite{mehrizi2018computer} reconstructs the 3D poses using Histogram Orientation Gradient (HoG) features from 2D multi-view cameras. The angle calculation are estimated at each frame after the 3D pose measurement by using OpenSim. 

\subsection{human abnormal behavior}

Paper \cite{morais2019learning} leverages the skeleton data from surveillance video to detect anomaly behavior. The novel Message-Passing Encoder-Decoder Recurrent Network models the movement patterns of normal people through global movement and local deformation. 

\subsection{SMPL model}

Paper \cite{zhang2020we} proposes a CVAE-based framework to predict human motion given the sparse marker sets on SMPL model. The authors claim that the sparse points on the body mesh also contains detailed human movement patterns which the skeleton data doesn't have.  


==> section/oldmethod.tex <==
\section{Methods}

Our goal is to perform lameness detection from the features extracted from raw mocap data. The feature descriptors are the model information obtained from the reconstructed 3D model sequence. Figure \ref{} shows our framework. In this section, we describe detailed information about the methods.

\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{image/framework.png}
\end{center}
   \caption{The whole framework.}
\label{fig:method_SMAL}
\end{figure}

\subsection{Dataset}
The Horse Treadmill Dataset is collected from an indoor treadmill by the University of Zurich \cite{rhodin2018vertical}. The soft tissues on the soles of horses are very sensitive. Therefore, the horses have been induced lameness by screwing a bolt against the sole, which creates "stone in the shoe" pain. This method can induce different levels of pain by controlling the depth of the bolt. The levels of pain are represented by numbers that larger number shows more pain the horse will feel. Some horses can adapt themselves to induction that they would behaves sound with pressure, which increases the difficulties for classification. In our experiments, we choose the data with larger levels of pain as possible since the horses have the instinct to hide their pains, and the lame patterns are easier observed with higher pain.

\subsection{Horse specific SMAL model}

Our horse-specific SMAL model $M(\beta, \theta, \gamma)$ is learned from 37 horse toys scan data. The topology of our horse-specific SMAL model is used from a 3D horse mesh downloaded from Sketchfab. There are a total of 36 segments on the body shown in Figure \ref{fig:method_SMAL}. The joints inside the model are calculated with the interfaces between two body segments.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{image/model_skeleton.png}
\end{center}
   \caption{The horse-specific SMAL model. 36 body segments are shown in different colors and the corresponding joint locations are shown in spheres in the same colors.}
\label{fig:method_SMAL}
\end{figure}

\subsection{Model Fitting}
We have two ways of fitting the model to the mocap data. The first one is to directly fit the model to the mocap data. Considering optimizing the accurate marker locations, we applied Mosh to the mocap data. 

The fitting process is adopted from SMAL model. And it minimizes an energy function for different cases with respect to model parameters $M(\beta, \theta, \gamma)$ and mocap data parameter $Mocap(r_m, t_m)$, where $r_m$ and $t_m$ are the rotation and translation of the mocap data, and camera parameters $C(f_c, k_c, rt_c, t_c)$, where $f_c=(f_x,f_y)$, $k_c$, $rt_c$, $t_c$ are the focal length, distortion coefficients, rotation, translation of the camera, respectively.

The perspective camera projection to the image plane is denoted as $\Pi(\cdot;C)$. $\cdot$ can be model $M$ that come with the projected model silhouette $\widehat{s}$, and any vertices on the model that results in the projection of the vertices. 


\paragraph{\ci{Energy term definition}}

A transformation between the mocap coordinate system and the camera coordinate system is performed for every sequence. The mocap data is updated as $T'$. More detail is shown below.
The $E_{mocap}$ is defined as the Mocap data loss:
\begin{small}
\begin{center}
\begin{equation}
E_{mocap}(\beta, \theta, \gamma) = \sum_{k} \rho (\left \| T'_{j} - M(\beta, \theta, \gamma)_{V_j} \right \|)
\label{equa:mocap loss}
\end{equation}
\end{center}
\end{small}

The $E_{sil}$, $E_{limit}$, $E_{\beta}$, $E_{\theta}$, $E_{cam}$  are defined in \cite{zuffi20173d}. 
The silhouette loss $E_{sil}$ utilizes a bi-directional distance between the projected silhouette $\widehat{S}$ and the ground truth silhouette $S$. More specifically, $E_{sil}$ = :
\begin{small}
\begin{center}
\begin{equation}
\sum_{x \in \widehat{S}} D_{S}(x)+ \sum_{x \in S} \rho(\underset{\widehat{x} \in \widehat{S}}{min}\left \| x - \widehat{x} \right \|)
\label{equa:silhouette loss}
\end{equation}
\end{center}
\end{small}

A set of angle ranges are manually set to limit the joint in each dimension. The limit loss is defined as $E_{limit}$ = :
\begin{small}
\begin{center}
\begin{equation}
max(\theta - \theta_{max},0) + max(\theta_{min} - \theta,0)
\label{equa:limit prior}
\end{equation}
\end{center}
\end{small}
where $\theta_{max}$ and $\theta_{min}$ are the maximum and minimum range of value in each dimension. 

The shape prior $E_{\beta}$ and pose prior $E_{\theta}$ are the squared Mahalanobis distance from the mean shape and mean pose. The gaussian with zero mean and variance is given by SMAL shape space and The gaussian with $\mu_{\theta}$ and $\sigma_{\theta}^{-1}$ is learned from all toy poses and pose sequences, respectively. 

\begin{small}
\begin{center}
\begin{equation}
E_{\beta} = (\beta - \mu_{\beta})^T \sigma_{\beta}^{-1} (\beta - \mu_{\beta})^T 
\label{equa:shape prior}
\end{equation}
\end{center}
\end{small}

\begin{small}
\begin{center}
\begin{equation}
E_{\theta} = (\theta - \mu_{\theta})^T \sigma_{\theta}^{-1}(\theta - \mu_{\theta})^T
\label{equa:pose prior}
\end{equation}
\end{center}
\end{small}

The camera loss $E_{cam}$ is to force $f_x$ equal to $f_y$.

\begin{small}
\begin{center}
\begin{equation}
E_{cam}(f) = \left \| f_x - f_y \right \|
\label{equa:camera update}
\end{equation}
\end{center}
\end{small}

\paragraph{Template generation}
\ci{template generation}
The specific subject has a fixed shape that is not changed for a short time. We apply the "one shape for one subject" strategy. The SMAL model is trained from toy scan data, which does not handle the soft-tissue. Thus, the template generated for each subject combines the silhouette to have more constraint on the shape, especially the belly. 

The data preparation for each subject is one image $I_s$, corresponding silhouette $S_s$, the corresponding Mocap data $T_s$, the corresponding 2D keypoints $K_s$ and each subject can have a basic template after the template generation. 

We adopt the energy terms from the SMAL model of fitting the model to images with 2D data $K_s$ and $S_s$, resulting in $\Phi_{2D}$. The problem of 2D information is the lack of depth information, which causes the wrong size of the final constructed subject.

To tackle this problem, we uses the results with 2D data input as the initialization for our model $M_{2D}$. Since the $T_s$ and the subject in $I_s$ are not in the same coordinate. The initialization can help $T_s$ to transform to the coordinate system where the model is. The transformation utilizes a pre-selected vertices on the model $V$ that represents the marker location. The transformed Mocap data $T_s'$ and the transformation matrix $Q$ is: 

\begin{small}
\begin{center}
\begin{equation}
\begin{aligned}
Q & = T_s^{\dagger} V  \\
T_s' & = M_{2D} Q + V_{origin}
\end{aligned}
\label{equa:transform}
\end{equation}
\end{center}
\end{small}

We update the camera focal length to make sure the projection is proper. We denote the energy function $F_{cam}$ to adjust the focal length. Specifically, let $x$ be the labeled 2D vertex, then: %and $V_{2d_j}^{m}$ be the pre-selected set of vertices on the model, then
\begin{small}
\begin{center}
\begin{equation}
F_{cam}(f) = \sum_{k} \rho (\left \| \Pi(T_{s'_j};f) - x \right \|)+ E_{cam}(f)
\label{equa:camera update}
\end{equation}
\end{center}
\end{small}
where $\rho$ is the Geman-McClure robust error function \cite{geman1987statistical}. 

The camera is fixed after it is updated, and our fitting objective function is:
\begin{small}
\begin{center}
\begin{equation}
F_{fit}(\Phi) = \sum_{\lambda \in {mocap, sil, \beta, \theta, limit}} \omega_{\lambda} E_{\lambda}(\cdot)
\label{equa:fitting}
\end{equation}
\end{center}
\end{small}


Since the translation and orientation of the model keeps optimizing in the fitting process, we re-transform the Mocap data and update the camera with respect to the optimized results. The whole fitting process follows an idea similar to Expectation Maximization. We keep iterative optimization three times. 


\paragraph{Fitting}
\ci{Simple Mosh}
For all the mocap sequences, our objective is defined as the weighted sum of the terms. Since we don't use video images in this case, we ignore the silhouette term.

\begin{small}
\begin{center}
\begin{equation}
F_{fit}(\Phi) = \sum_{\lambda \in {mocap, \beta, \theta}} \omega_{\lambda} E_{\lambda}(\cdot)
\label{equa:fitting2}
\end{equation}
\end{center}
\end{small}

The body shape is considered to be time-invariant and can be the same for a set of sequences from the same subject. We consider finetuning on the body shape obtained from the first stage. We randomly choose 20 frames inside a sequence for each subject and fine-tune on that body shape in order to have a better shape. Once the finetune is done, the optimization does not include the shape input.


\paragraph{Mosh}
\ci{Mosh not done}
The other is using Mosh.

\subsection{Lameness detection}
To perform lameness detection. ST-GCN is applied to both the mocap data and the 3D model sequence. 

\subsection{Feature extraction}


\paragraph{Mocap data}

Most of the markers are put on the rigid joints according to anatomy. We assume to form the skeleton using the markers. The skeleton graph designed for ST-GCN is based on the marker shown in Figure \ref{fig:mocap_skeleton}. The marker positions are the input to ST-GCN.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{image/mocap_graph.png}
\end{center}
   \caption{The defined graph for ST-GCN using mocap data.The number indicates the node and the red line indicates the edge between node. }
\label{fig:mocap_skeleton}
\end{figure}

\paragraph{Model sequence}

The 3D model contains the joints including the relative rotation between the body segment and its parent segments and the 3D joint locations. We form the skeleton graph using these joints' information. The skeleton graph designed for ST-GCN is based on the model sequence shown in Figure \ref{fig:model_skeleton}. The input to ST-GCN are the relative rotations, that is the pose parameters. \ci{input could be the 3D joint locations or the marker location on the body model}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\linewidth]{image/smal_graph.png}
\end{center}
   \caption{The defined graph for ST-GCN using model sequence. The number indicates the node. The red solid line indicates the edge between node. The dotted lines indicates the unused edges. }
\label{fig:model_skeleton}
\end{figure}

